Gravitational Lenses in UNIONS and Euclid (GLUE) I: A Search for Strong Gravitational Lenses in UNIONS with Subaru, CFHT, and Pan-STARRS Data

We present the results of our pipeline for discovering strong gravitational lenses in the ongoing Ultraviolet Near-Infrared Optical Northern Survey (UNIONS). We successfully train the deep residual neural network (ResNet) based on CMU-Deeplens architecture, which is designed to detect strong lenses in ground-based imaging surveys. We train on images of real strong lenses and deploy on a sample of 8 million galaxies in areas with full coverage in the g, r, and i filters, the first multi-band search for strong gravitational lenses in UNIONS. Following human inspection and grading, we report the discovery of a total of 1346 new strong lens candidates of which 146 are grade A, 199 grade B, and 1001 grade C. Of these candidates, 283 have lens-galaxy spectroscopic redshifts from the Sloan Digital Sky Survey (SDSS) and an additional 297 from the Dark Energy Spectroscopic Instrument (DESI) Data Release 1 (DR1). We find 15 of these systems display evidence of both lens and source galaxy redshifts in spectral superposition. We additionally report the spectroscopic confirmation of seven lensed sources in highquality systems, all with z > 2.1, using the Keck Near-Infrared Echelle Spectrograph (NIRES) and Gemini Near-Infrared Spectrograph (GNIRS).

==> sections/TS-tbl.tex <==


\begin{deluxetable}{lc|cc|cc|cc}[h]
\centering

% \tabletypesize{\small}
\tablecaption{Training Sample Counts\label{tab:training-sample}}
\tablehead{& \multicolumn{2}{|c}{\textbf{Training}}        & \multicolumn{2}{|c}{\textbf{Validation}}      & \multicolumn{2}{|c}{\textbf{Total}}            } 
 \startdata
 \hline
 & \multicolumn{1}{|c|}{~~lens~~} & non-lens & \multicolumn{1}{|c|}{~~lens~~} & non-lens & \multicolumn{1}{|c|}{~~lens~~} & non-lens \\ \hline
\textit{\textbf{gri}} & \multicolumn{1}{|c|}{541}  & 25619     & \multicolumn{1}{|c|}{232}  & 10980     & \multicolumn{1}{|c|}{773}  & 36599     \\ 
\enddata
\end{deluxetable}


% \begin{deluxetable*}{lccccccc}
% \centering

% \tablewidth{30pt}
% \tabletypesize{\small}
% \tablecaption{UNIONS Coverage\label{tab:UNIONS-coverage}}
% \tablehead{\colhead{Region} & \colhead{\textit{u}} & & \colhead{\textit{r}} & &  \colhead{\textit{i}} & \colhead{\textit{uri}}}
% \startdata
% South Galactic Cap  &2850& &483&&0& 0\\
% North Galactic Cap &3827& &2680&  &3415&2183\\
%  \hline
%  Total&  6677& &3163& &3415&2183\\ 
% \enddata
% \tablecomments{There is available \textit{i}-band data in the South Galactic Cap from an earlier processing. To avoid confusion between different data formats we opt to exclude it for now. All values are given in square degrees.}
% \end{deluxetable*}

==> sections/abstr.tex <==
We present the results of our pipeline for discovering strong gravitational lenses in the ongoing Ultraviolet Near-Infrared Optical Northern Survey (UNIONS). We successfully train the deep residual neural network (ResNet) based on  \texttt{CMU-Deeplens} architecture, which is designed to detect strong lenses in ground-based imaging surveys. We train on images of real strong lenses and deploy on a sample of 8 million galaxies in areas with full coverage in the \textit{g}, \textit{r}, and \textit{i} filters, the first multi-band search for strong gravitational lenses in UNIONS. Following human inspection and grading, we report the discovery of a total of \totalprelim new strong lens candidates of which \gradeAfinal are grade A, \gradeBfinal grade B, and \gradeCfinal grade C. Of these candidates, 283 have lens-galaxy spectroscopic redshifts from the Sloan Digital Sky Survey (SDSS) and an additional 297 from the Dark Energy Spectroscopic Instrument (DESI) Data Release 1 (DR1). We find 15 of these systems display evidence of both lens and source galaxy redshifts in spectral superposition.
We additionally report the spectroscopic confirmation of seven lensed sources in high-quality systems, all with $z>2.1$, using the Keck Near-Infrared Echelle Spectrograph (NIRES) and Gemini Near-Infrared Spectrograph (GNIRS).

==> sections/deploy.tex <==
As described in Section~\ref{sec:deployment-strat}, we will deploy the trained CNN to all skycells in UNIONS with full \textit{uri} data. The CNN will predict probabilities for cutouts centered on galaxies included in the DESI Legacy Surveys source catalog. While trained on GPUs, CNN predictions can be made on a CPU at a rate of $\sim65$ images per second ($\sim10\times$ slower than on a GPU). However, access to a large number of CPU nodes via the IPP cluster will greatly reduce the total time for a full deployment. Predictions for all $10^7$ images are projected to take $\sim45$ hours on a single CPU. This of course neglects overheads including input/output (IO) times, but shows that CNN speed will not cause bottlenecks at the time of deployment. When considering parallelization across dozens of CPU nodes, runtime for a full CNN deployment is of no concern. 

While we are not yet prepared to conduct a full deployment, we have completed small-scale test deployments. Here we will present the results of deployment on a single skycell in UNIONS. The randomly selected skycell is shown in Figure~\ref{fig:sc170}. Over-plotted are red markers corresponding to the 457 objects from the DESI source catalog which fall within this skycell. Figure~\ref{fig:deploy-probs} shows the distribution of predicted probabilities for each of the object cutouts. Note that only 3\% (13/457) of the cutout images received a probability~$>$~0.1. For full deployment, rigorous inspection and grading of CNN recommendations (above a given probability threshold) is necessary to distinguish high-quality strong lens candidates. Given we are only reporting results for deployment on a single skycell, inspection of images across a wide range of probabilities (including $<0.1$) has been conducted. Our primary goal for this paper is not to find strong lens candidates but rather assess CNN performance for deployment. 


Figure~\ref{fig:high-prob} shows four hand-selected examples of images which received a probability $>0.1$. These are representative of typical false positives which appear often in searches for strong lenses. Rows one and two show ``red-near-blue" configurations. Strong lenses will typically have orange-red colored elliptical galaxy lenses and most often blue lensed images or arcs. Thus, observing that the CNN gives a relatively high probability to ``red-near-blue" configurations is not surprising. Row three contains an over-saturated star. No images containing saturated stars were \textit{intentionally} added to the training sample. Adding such images may help the CNN to handle cases such as this in future deployments, however the consequences of this are not known. An alternative may be to include a larger number of non-lenses in the training sample, increasing the chance for images containing saturated stars to be included. The last row shows a clear example of a spiral galaxy. This again is a ``red-near-blue" configuration but also can be confusing due to spiral morphology. Lensed sources typically appear as arc-like structures which can easily be confused with spiral arms and vice-versa. Observing potential contaminants from small-scale deployments such as this are highly valuable, in particular when it comes to assessing the quality of the training sample. From these results, it seems reasonable to increase the number of non-lenses in the training sample. Growing the training sample should be done incrementally in order to closely track how model performance changes. Constructing the training sample to enable the CNN to learn what a lens is not should be viewed as the top priority when the lens sample is fixed, as it is here. 
% \vspace{0.5cm}

With the expectation that one in every $10^4$ galaxies acts as a lens and with $\sim500$ galaxies per skycell, it is reasonable to expect $\sim$1 strong lens for every 20 skycells, 5\% probability. Despite only deploying on a single skycell, we have identified one strong lens candidate, shown in Figure~\ref{fig:candidate}. It received a probability of exactly 0.100 and would thus be classified as a lens at a hypothetical threshold of 0.1 (inclusive). The CFIS \textit{r}-band shows signs of a possible arc-like structure to the north-east of the presumptive lens galaxy at the center of the image. Its morphology appears to be distinct from a spiral arm due in part to the separation between it and presumptive lens galaxy (i.e. it does not clearly ``spiral" inward). Additionally, the low surface brightness observed in the \textit{r}-band is within expectation for a strongly lensed arc. There is not much color information to aid in classification for this arc as it is only clearly present in the \textit{r}-band image. This system does not currently have \textit{g}-band data from WHIGS, though the color information, image quality, and signal-to-noise provided by WHIGS would certainly aid in classification. While showing evidence of strong lensing, this candidate system would likely be classified with moderate to low confidence. Systems such as this will require either high-resolution imaging or spectroscopy to confirm its nature (discussed in Section~\ref{sec:future}) but will nonetheless be reported as candidates when our work is published. 





% \begin{itemize}
%     \item discuss deployment strategy
%     \begin{itemize}
%         \item skycell breakdown--multi cpu on IPP--total runtime est?
%     \end{itemize}
%     \item show deployment results--any lenses if found 
% \end{itemize}

==> sections/deployment-strat.tex <==
Following training (the results of which are discussed in Section~\ref{sec:training}), the CNN model is frozen and deployed on UNIONS image data. In this process we will again use the DESI Legacy Surveys object catalog of galaxies brighter than 20th mag. in \textit{z}-band. Stamp-sized cutouts ($160\times160$ pixels) centered on each of the $\sim10^7$ objects will be produced and fed as the input to the CNN. Each image will receive a predicted probability between 0 and 1, corresponding to how likely the image is to contain a strong lensing system. In this case an image above a given probability threshold is classified as a lens. Typically, for binary classification tasks, a probability threshold of 0.5 is set to distinguish between classes. However, this threshold can be adjusted for different goals. For instance one can prioritize completeness or purity by setting a lower or higher threshold respectively. Here, purity = precision = TP/(TP + FP) and completeness = TP/(TP + FN) where TP is true positives (correctly classified lenses), FP is false positives (non-lenses classified as lenses), and FN is false negatives (lenses classified as non-lenses). Any image which receives a probability above the given threshold will be referred to as ``recommendations". Recommendations will then be subject to human inspection where the final determination will be made. This is necessary because it is extremely difficult to achieve prefect precision, especially for a difficult classification task such as this. \citet{storfer2022a} achieved the highest reported precision for a strong lens search, finding $\sim$1 strong lens candidate for every 25 CNN recommendations. They also report the most strong lensing candidates in a single search (1895  total, 1512 new). This was achieved with a much larger training sample in a more homogeneous survey. Their probability threshold was determined with the goal of balancing precision and completeness. For this search, we opt to prioritize precision over completeness. The current limitations of the training sample, and thus training performance, will likely require a high probability threshold to maintain a high precision. Final determination of the probability threshold will be made just prior to deployment and will be largely based on the performance of the latest trained CNN model (see Section~\ref{sec:training}).

\input{sections/TS-tbl}
% \begin{minipage}{0.95\textwidth}
% \vspace{-1.5cm}
% \makebox[\textwidth][c]{
%   \includegraphics[keepaspectratio=true,scale=0.8]{figures/filter_frac.png}}
%   \captionsetup{font=footnotesize}
%   \vspace{-0.8cm}
% \captionof{figure}{\footnotesize All combinations of filter coverage in the UNIONS data used in this work. Fractions are shown for three sets of sources; (1) data across the entire UNIONS footprint in blue, (2) data for the sources in the DESI catalog in green, and (3) data for the full set of 517 lenses in red. (1) has a significant area with unique \textit{u}-band coverage in the South Galactic Cap. (2) is a reflection of the area in the North Galactic Cap. (3) does not have the same fraction for each filter combination as (2) because the location of known lenses is not uniformly distributed across the survey (many lenses were discovered in the HSC-SSP).}
% \label{fig:filter-data}
% \vspace{0.25cm}

% \end{minipage}


The vast amounts of data in UNIONS requires strategic deployment of the CNN to ensure computational efficiency, particularly in terms of runtime. Deployment will be conducted on central processing unit (CPU) nodes available to us on the Pan-STARRS Image Processing Pipeline (IPP) cluster. We have consolidated the UNIONS \textit{uri} data in a central location within the cluster for ease of access. The image data is subdivided into small regions called ``skycells" which are $0.5\times0.5^{\circ}$ in size. There are a total of 12870 skycells with \textit{uri} coverage. With a strategy which we refer to as ``on-the-fly" deployment, cutouts will be produced for all objects in a given skycell and held in memory during the deployment process. After all images for a skycell are processed by the CNN, only those which receive a probability above the threshold will be saved to storage at which point all other images will be removed from memory. All predicted probabilities will be saved for future reference. This process will be highly parallelized by distributing skycells to available CPU nodes.

==> sections/fut_followup.tex <==
UNIONS provides a unique opportunity to discover a large number of lenses prior to the first dedicated, high-resolution, optical and near-IR space-based survey telescope, \textit{Euclid}. By knowing the positions of strong lens candidates {\em a priori}
, we can immediately confirm their nature as \textit{Euclid} data is processed. We expect $\mathcal{O}(10^3)$ discoverable strong lenses in UNIONS \citep[see][]{collett2015a} and \textit{Euclid} will provide high-resolution imaging for all of them. In addition to confirmation, \textit{Euclid} imaging can also be used, alongside spectroscopic redshifts, to produce accurate strong lens models for these systems. This is the motivation for my thesis work. 
Discovering a large sample of strong lenses in UNIONS will enable statistical studies and even make it possible to down-select to an optimal set of lenses for a given science goal. In particular, we will target galaxy-scale strong lenses with simple morphologies. Galaxy-scale lenses are in general the simplest to model and this simplicity motivates a variety of science including but not limited to: (1) mass measurements of elliptical galaxies at cosmological distances, including mapping the distribution of dark matter in such galaxies, (2) probing low-mass dark matter halos ($<10^9$M$_\odot$) which can perturb lensed images/arcs, (3) studies of high-redshift source galaxies enabled by strong lensing magnification, and (4) measurements of cosmological parameters such as the Hubble constant ($H_0$) via strongly lensed transients. 
 
Again, all of this science and more is only possible if accurate lens models can be produced. In order to conduct statistical studies, models must be produced for a large number of strong lenses. Recent developments in lens modeling software have greatly improved the efficiency of lens modeling. For example, GIGA-Lens \citep{gu2022a} takes advantage of automatic differentiation and massive parallelization on GPUs. It is capable of modeling the hundreds of systems that will be observed by Euclid. This will be the largest scale modeling effort of strong lenses to date. 
 
% \begin{itemize}
%     \item search in single band VIS 
%     \begin{itemize}
%         \item smaller r\_E, higher z (collett+ 2015)
%         \item multi-band GB better than single-band SB (metcalf+ 2018)
%     \end{itemize}
%     \item high-res follow-up for lenses found in UNIONS
%     \begin{itemize}
%         \item THESIS WORK--largest scale modeling effort
%     \end{itemize}
    
% \end{itemize}

==> sections/fut_search.tex <==
Upon completion, UNIONS will be unrivaled in its coverage of the North Galactic Cap. In terms of potential for finding strong lenses as a ground-based survey, UNIONS will only be rivaled by the Vera C. Rubin Observatory's upcoming Legacy Survey of Space and Time (LSST). \citet{metcalf2018a} showed that in a search for strong lenses, regardless of search method, classification with multi-band, ground-based imaging consistently outperformed single-band space-based imaging. This is because color information is critically important in classification, even at the expense of resolution or signal-to-noise. Therefore, continuing the effort to search for lenses in UNIONS, especially after its completion, will likely yield a high number of quality systems. Lens searches in \textit{Euclid} will also prove to be highly valuable due to its depth and incredible image quality, though a search will not be possible until a considerable amount of survey data is collected (at least 2-3 years from now). 
% While the VIS filter has much better resolution than the infrared (IR) filters, as stated, the additional color information is extremely helpful. 
Searches for lenses exclusively using the VIS filter (which has the highest resolution) will be able to probe a largely unique population of strong lenses down to very small Einstein radii \citep[see][]{collett2015a}. Comparing the selection function of lenses in UNIONS vs \textit{Euclid} will likely shed light on the intrinsic biases within search methodologies. Additionally, we could consider combining data from UNIONS and \textit{Euclid} in a search. This would likely increase detection rates over either individual survey.
% In addition to searches for galaxy-galaxy lenses (where an ordinary galaxy acts as the source), we may also consider conducting a search for galaxy-quasar lensing systems in UNIONS and Euclid. This can either be done as a catalog search using an auto-correlation algorithm \citep[e.g.][]{dawes2022a} or with a machine learning based approach. Lensed quasars are powerful probes of the cosmic expansion rate (H$_0$), similar 

% \begin{itemize}
%     \item search upon survey completetion 
%     \item lensed quasar search
%     \item macro-lens modeling (g+r band)
%     \item spectroscopic follow-up (DESI + NIRES/other)
%     \item lensed SN (?) -- just to be sure
% \end{itemize}

==> sections/future.tex <==
We have managed to train our CNN to a satisfactory level and perform a small-scale deployment. There are many aspects of our CNN training which can be improved, outlined in \S~\ref{sec:alt-search}. In \S~\ref{sec:search-future} we discuss the potential of future searches for strong lenses in both UNIONS and Euclid and \S~\ref{sec:followup-future} describes future follow-up efforts of our newly discovered strong lens candidates.

% Work done for this project has and will directly contribute to the goals of my thesis work. This is the first of a series of papers which will focus on strong lensing science in UNIONS and the \textit{Euclid} survey. 


